Optimal Continuous Time Markov Decisions

In the context of Markov decision processes running in continuous time, one of the most intriguing challenges is the efficient approximation of finite horizon reachability objectives. A multitude of sophisticated model checking algorithms have been proposed for this. However, no proper benchmarking has been performed thus far. This paper presents a novel and yet simple solution: an algorithm originally developed for a restricted subclass of models and a subclass of schedulers can be twisted so as to become competitive with the more sophisticated algorithms in full generality. As the second main contribution, we perform a comparative evaluation of the core algorithmic concepts on an extensive set of benchmarks varying over all key parameters: model size, amount of non-determinism, time horizon, and precision.

==> figures/DynamicPM_Early_Fanout_t=5_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeEF, shift={($(scopeES.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=1000, xmin=2, xmax=7,
		axis y line=left,axis x line=bottom,
		xlabel={fanout},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (2,0.011524) (3,0.045538) (4,0.108184) (5,0.266937) (6,2.894218) (7,7.895513) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (2,3.400025) (3,53.142012) (4,715.328930) (5,715.328930) (6,900) 
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) node[above left]{timeout};
	\end{semilogyaxis}
\end{scope}


==> figures/DynamicPM_Early_States_t=5_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=50, xmin=71, xmax=800,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]


        	\addplot coordinates {
		 (71,0.039736) (117,0.074881) (175,0.119846) (245,0.174154) (327,0.2395) (421,0.312766) (527,0.394716) (645,0.488449) (775,0.598061) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (71,0.002383) (117,0.004076) (175,0.006195) (245,0.00881) (327,0.012447) (421,0.016302) (527,0.019929) (645,0.028274) (775,0.030609) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (71,3.44832) (117,5.53543) (175,8.41893) (245,11.7507) (327,15.7146) (421,20.3964) (527,25.289) (645,30.9429) (775,37.5046) 
	};
	\addlegendentry{\ESS-1}

%		\addplot (\x, {900});
	\end{semilogyaxis}
\end{scope}

==> figures/DynamicPM_Early_Time_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeET] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10000, xmin=2, xmax=20,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (1,0.003576) (2,0.010000) (3,0.018323) (4,0.028319) (5,0.039284) (6,0.052089) (7,0.065520) (8,0.079471) (9,0.095477) (10,0.117296) (25,0.439033) (50,1.245424) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (1,0.001384) (2,0.001200) (3,0.002093) (4,0.002983) (5,0.002409) (6,0.002581) (7,0.002752) (8,0.002851) (9,0.002819) (10,0.002956) (25,0.002902) (50,0.000703) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (1,0.136736) (2,0.548123) (3,1.220736) (4,2.176052) (5,3.435246) (6,4.898032) (7,6.658965) (8,8.701619) (9,11.116290) (10,15.680111) (25,89.047621) (50,347.398979) 
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) node[above left]{timeout};		
		
	\end{semilogyaxis}
\end{scope}

==> figures/DynamicPM_Late_Fanout_t=10_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLF, shift={($(scopeLS.south)-(1.5cm, 4cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10000,xmin=4, xmax=7,
		axis y line=left,axis x line=bottom,
		xlabel={fanout},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
		
        	\addplot coordinates {
		 (2,0.303772) (3,2.795513) (4,26.278493) (5,374.997998) (6,1847.070765) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (2,0.299287) (3,1.955222) (4,15.204816) (5,104.520787) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (2,0.367127) (3,1.563685) (4,5.815430) (5,13.649495) (6,86.194776) (7,685.219984) (8,2366.814896) (9,6000) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (2,0.184468) (3,0.968808) (4,3.375684) (5,7.124896) (6,44.640084) (7,361.542365) (8,1302.093573) (9,3600) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (2,0.325768) (3,1.146001) (4,5.390761) (5,5.429314) (6,152.827810) (7,1121.068594) 
	};
	\addlegendentry{\GUS}


%		\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}


==> figures/DynamicPM_Late_States_t=5_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLS, shift={($(scopeLE.south)-(1.5cm, 4cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=1800,xmin=412, xmax=370000,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]


       	\addplot coordinates {
		 (412,1.01745) (1732,4.73336) (4564,12.9074) (9484,32.987) (17068,63.906) (27892,113.182) (42532,207.887) (61564,313.285) (85564,395.98) (115108,546.642) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (412,3.4274) (1732,16.5274) (4564,47.0466) (9484,142.816) (17068,366.165) (27892,752.685) (42532,1187.01) (61564,1380.88) (85564,1786.7) (115108,2572.9) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (412,0.916779) (1732,4.4658) (4564,12.2214) (9484,25.0078) (17068,45.8823) (27892,75.6493) (42532,124.844) (61564,193.046) (85564,290.798) (115108,390.367) (150772,518.852) (193132,674.284) (242764,864.088) (300244,1077.91) (366148,1325.43) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (412,0.620255) (1732,2.5808) (4564,6.97909) (9484,14.3163) (17068,25.1755) (27892,41.8781) (42532,71.2837) (61564,111.067) (85564,166.958) (115108,219.797) (150772,289.152) (193132,378.479) (242764,484.113) (300244,602.43) (366148,742.869) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (412,0.722391) (1732,5.41824) (4564,14.9316) (9484,31.6584) (17068,57.5409) (27892,94.8701) (42532,152.665) (61564,234.312) (85564,365.366) (115108,512.976) (150772,686.858) (193132,884.066) (242764,1126.4) (300244,1392.39) (366148,1717.49) 
	};
	\addlegendentry{\GUS}

%		\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}


==> figures/DynamicPM_Late_Time_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLT, shift={($(scopeET.east)+(2cm, -1.5cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0.01,ymax=10,xmin=1, xmax=50,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
        	\addplot coordinates {
		 (1,0.115122) (2,0.128746) (3,0.144487) (4,0.161503) (5,0.180539) (6,0.200578) (7,0.222506) (8,0.245606) (9,0.269138) (10,0.293782) (25,0.739220) (50,1.696397) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (1,0.126304) (2,0.163834) (3,0.211848) (4,0.269554) (5,0.334540) (6,0.407334) (7,0.484722) (8,0.568227) (9,0.657885) (10,0.753349) (25,2.671691) (50,7.340338) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (1,0.033602) (2,0.048912) (3,0.118177) (4,0.118008) (5,0.114185) (6,0.132302) (7,0.154579) (8,0.177054) (9,0.199833) (10,0.222690) (25,0.577874) (50,1.198344) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (1,0.028710) (2,0.043871) (3,0.104337) (4,0.106107) (5,0.101098) (6,0.108094) (7,0.127080) (8,0.145096) (9,0.161885) (10,0.181133) (25,0.459929) (50,0.981335) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
                 (1,0.026784) (2,0.035116) (3,0.085305) (4,0.169587) (5,0.074771) (6,0.082689) (7,0.099628) (8,0.116320) (9,0.133247) (10,0.151317) (25,0.429065) (50,0.086418)
	};
	\addlegendentry{\GUS}


%		\addplot (\x, {900}) node[above left]{timeout};		
	\end{semilogyaxis}
\end{scope}


==> figures/ErlangStages_Early_Precision_t=7.tex <==
\begin{scope}[local bounding box=scopeEE, shift={($(scopeET.south)-(1.6cm, 4cm)$)}]
	\begin{loglogaxis}[
		x dir=reverse,
		ymin=0,ymax=10000,xmin=1e-10, xmax=0.001,
		axis y line=left,axis x line=bottom,
		xlabel={precision},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.001,0.059938) (0.0001,0.123340) (1e-05,0.373132) (1e-06,1.174689) (1e-07,3.713395) (1e-08,11.757933) (1e-09,37.078337) (1e-10,900) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.001,0.006171) (0.0001,0.030248) (1e-05,0.203103) (1e-06,2.534103) (1e-07,21.652867) (1e-08,177.481881) (1e-09,2868.295806) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.001,6.603859) (0.0001,66.405158) (1e-05,666.493905) (1e-06,900) (1e-07,900) (1e-08,900) (1e-09,900) (1e-10,900) 
	};
	\addlegendentry{\ESS-1}


%	\addplot (\x, {900});
	
	\end{loglogaxis}

\end{scope}


==> figures/ErlangStages_Early_States_t=20_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0.001,ymax=1000, xmin=204, xmax=2010,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]


        	\addplot coordinates {
		 (204,1.157) (404,2.33225) (604,3.61824) (804,4.8401) (1004,5.91943) (1204,7.13023) (1404,8.28055) (1604,9.47915) (1804,10.6384) (2004,11.8051) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (204,0.001366) (404,0.002625) (604,0.003985) (804,0.005335) (1004,0.006733) (1204,0.008033) (1404,0.010448) (1604,0.010783) (1804,0.012008) (2004,0.013407) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (204,751.215) (404,900) 
	};
	\addlegendentry{\ESS-1}

	


%		\addplot (\x, {900});
	\end{semilogyaxis}
\end{scope}


==> figures/ErlangStages_Late_States_t=20_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLS, shift={($(scopeLE.south)-(1.5cm, 4cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=1260,xmin=1004, xmax=30010,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
		
		
        	\addplot coordinates {
		 (1004,55.2202) (2004,108.5) (3004,119.146) (4004,214.079) (5004,196.612) (10004,395.236) (15004,793.907) (20004,1075.76) (25004,1035.97) (30004,1257.37) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (1004,254.137) (2004,503.046) (3004,663.874) (4004,1027.05) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (1004,0.057252) (2004,0.101773) (3004,0.149016) (4004,0.193918) (5004,0.236437) (10004,0.470574) (15004,0.701789) (20004,0.942491) (25004,1.19945) (30004,1.44937) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (1004,0.09098) (2004,0.147459) (3004,0.207488) (4004,0.260779) (5004,0.317454) (10004,0.601874) (15004,0.901181) (20004,1.22486) (25004,1.52822) (30004,1.85502) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (1004,0.005986) (2004,0.010484) (3004,0.015359) (4004,0.020386) (5004,0.026702) (10004,0.05128) (15004,0.079254) (20004,0.10429) (25004,0.133768) (30004,0.164681) 
	};
	\addlegendentry{\GUS}

%		\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}


==> figures/FTWC_Early_Precision_t=10.tex <==
\begin{scope}[local bounding box=scopeEE, shift={($(scopeET.south)-(1.6cm, 4cm)$)}]
	\begin{loglogaxis}[
		x dir=reverse,
		ymin=1e-4,ymax=10000,xmin=1e-10, xmax=0.001,
		axis y line=left,axis x line=bottom,
		xlabel={precision},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
       	\addplot coordinates {
		 (0.001,0.000771) (0.0001,0.000737) (1e-05,0.000738) (1e-06,0.000848) (1e-07,0.000829) (1e-08,0.000919) (1e-09,0.000971) (1e-10,0.001717) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.001,2.114733) (0.0001,21.497532) (1e-05,212.016519) (1e-06, 900) 
	};
	\addlegendentry{\ESS-1}


%	\addplot (\x, {900});
	
	\end{loglogaxis}

\end{scope}


==> figures/FTWC_Early_States_t=10_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{loglogaxis}[
		ymin=0.001,ymax=10, xmin=110, xmax=600000,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (110,0.003801) (818,0.019009) (2770,0.035978) (10130,0.089273) (38674,0.507857) (151058,2.10152) (597010,8.61953) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (110,20.6284) (818,160.351) (2770,546.63) (10130,900) (38674,900) (151058,900) 
	};
	\addlegendentry{\ESS-1}

%		\addplot (\x, {900});
	\end{loglogaxis}
\end{scope}


==> figures/FTWC_Early_Time_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeET] 
	\begin{semilogyaxis}[
		ymin=0.1,ymax=1000, xmin=5, xmax=50,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (5,0.966058) (10,0.965806) (15,0.965923) (20,0.965811) (25,0.965752) (30,0.965585) (35,0.965593) (40,0.965803) (45,0.965749) (50,0.965804) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (5,8.613291) (10,35.355456) (15,95.908338) (20,189.064500) (25,303.458200) (30,437.539959) (35,608.595356) (40,813.188380) (45,900)
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) ;		
		
	\end{semilogyaxis}
\end{scope}


==> figures/FTWC_Late_Precision_t=100.tex <==
\begin{scope}[local bounding box=scopeFLE, shift={($(scopeELE.south)-(1.5cm, 4cm)$)}] 		
	\begin{loglogaxis}[
			x dir=reverse,
			ymin=0,ymax=10000,xmin=1e-10, xmax=1e-03,
			axis y line=left,axis x line=bottom,
                        xlabel={\hh{todo}},
                        ylabel={},
                        height=5cm,
                        width=5cm,
			legend style={rounded corners,at={(0.9,0.9)}},
			grid style = {
				dash pattern = on 0.05mm off 1mm,
				line cap = round,
				black,
				line width = 0.5pt
			},
			cycle list name=latelist
		]

                	\addplot coordinates {
		 (0.001,59.727128) (0.0001,134.853157) (1e-05,309.601111) (1e-06,671.565297) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (0.001,109.366033) (0.0001,453.371657) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (0.001,0.879395) (0.0001,1.150185) (1e-05,1.499197) (1e-06,1.902048) (1e-07,2.579828) (1e-08,4.688639) (1e-09,19.925879) (1e-10,156.925391) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (0.001,1.198304) (0.0001,1.544035) (1e-05,1.985683) (1e-06,2.537170) (1e-07,3.292561) (1e-08,5.271303) (1e-09,18.337653) (1e-10,131.898810) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (0.001,0.037446) (0.0001,0.039166) (1e-05,0.039263) (1e-06,0.040492) (1e-07,0.041140) (1e-08,0.042376) (1e-09,0.042259) (1e-10,0.042360) 
	};
	\addlegendentry{\GUS}


		
%		\addplot (\x, {900});
		
	\end{loglogaxis}
		
\end{scope}

==> figures/GFS_Early_Precision_t=1.tex <==
\begin{scope}[local bounding box=scopeEE, shift={($(scopeET.south)-(1.6cm, 4cm)$)}]
	\begin{loglogaxis}[
		x dir=reverse,
		ymin=0,ymax=10000,xmin=1e-10, xmax=0.001,
		axis y line=left,axis x line=bottom,
		xlabel={precision},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.001,151.179615) (0.0001,482.835749) (1e-05,900)
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.001,0.059516) (0.0001,0.057612) (1e-05,0.059649) (1e-06,0.063099) (1e-07,0.327824) (1e-08,2.895942) (1e-09,7.070584) (1e-10,16.741143) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.001,7200)
	};
	\addlegendentry{\ESS-1}


%	\addplot (\x, {900});
	
	\end{loglogaxis}

\end{scope}


==> figures/GFS_Early_States_t=1_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{loglogaxis}[
		ymin=0,ymax=2000, xmin=5000, xmax=15300,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]


       	\addplot coordinates {
		 (2507,475.863) (2507,477.798) (2508,476.907) (5557,1939.26) (5557,1940.2) (5558,1949.55) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (2507,0.056671) (2507,0.058117) (2508,0.058283) (5557,0.166943) (5557,0.170132) (5558,0.174672) (9807,0.4008) (9807,0.41516) (9808,0.434536) (15257,0.844887) (15257,0.826102) (15258,0.856401) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (2507,1200) 
	};
	\addlegendentry{\ESS-1}



%		\addplot (\x, {900});
	\end{loglogaxis}
\end{scope}


==> figures/GFS_Early_Time_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeET] 
	\begin{semilogyaxis}[
		ymin=0,ymax=2000, xmin=2, xmax=10,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.5,168.676678) (1,482.935839) (1.5,875.897546) (2,1349.716234) (2.5,1918.650420) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.5,0.032472) (1,0.039280) (1.5,0.043766) (2,0.047973) (2.5,0.050779) (3,0.054531) (3.5,0.061801) (4,0.069657) (4.5,0.077315) (5,0.084664) (5.5,0.091815) (6,0.099518) (6.5,0.106709) (7,0.114759) (7.5,0.121603) (8,0.128646) (8.5,0.136254) (9,0.143436) (9.5,0.150005) (10,0.158191) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.1,1105.683313) 
	};
	\addlegendentry{\ESS-1}

	\addplot coordinates {
		 (0.5, 900)
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) node[above left]{timeout};		
		
	\end{semilogyaxis}
\end{scope}


==> figures/GFS_Late_Time_e=1e-08.tex <==
\begin{scope}[local bounding box=scopeGLT, shift={($(scopeQLT.east)+(1cm, -1.5cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10000,xmin=1, xmax=50,
		axis y line=left,axis x line=bottom,
		xlabel={\hh{todo, plot needs revision}},
		ylabel={},
		height=5cm,
		width=5cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
        	\addplot coordinates {
		 (1,900) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (1,900) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (1,11.3326) (2,24.7395) (3,38.9221) (4,53.9826) (5,69.506) (6,85.5927) (7,102.037) (8,118.916) (9,136.042) (10,153.34) (25,423.761) (50,716.866) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (1,10.0222) (2,21.1944) (3,33.0529) (4,45.6707) (5,58.6368) (6,71.8868) (7,85.4284) (8,99.3058) (9,113.414) (10,127.884) (25,349.183) (50,589.43) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
(1,23.9047) (2,9.97675) (3,0.411045) (4,54.3669) (5,31.1371) (5.1,13.5269) (5.2,5.44268) (5.3,2.02372) (5.4,5.88321) (5.5,79.1312) (5.6,81.0806) (5.7,6.23368) (5.8,0.743626) (5.9,0.757196) (6,0.764428) (6.1,2.43246) (6.2,17.4202) (6.3,41.9022) (6.4,94.238) (6.5,43.2158) (6.6,3.07111) (6.7,0.853101) (6.8,0.856467) (6.9,7.97852) (7,224.163) (7.1,48.0254) (7.2,231.724) (7.3,109.023) (7.4,21.7419) (7.5,8.74951) (7.6,3.56379) (7.7,9.09223) (7.8,532.279) (7.9,260.658) (8,547.055) (8.1,264.892) (8.2,125.555) (8.3,57.2064) (8.4,26.3822) (8.5,10.5032) (8.6,10.7711) (8.7,10.6565) (8.8,61.9596) (8.9,611.723) (9,139.577) (9.1,28.8813) (9.2,11.4076) (9.3,1.13958) (9.4,1.32851) (9.5,4.47242) (9.6,30.1785) (9.7,670.394) (9.8,676.28) (9.9,327.297) (10,156.133) (10.1,72.1047) (10.2,31.9896) (10.3,13.498) (10.4,5.29746) (10.5,1.3343) (10.6,1.35597) (10.7,1.51369) (10.8,1.43715) (10.9,1.44273) (11,1.72355) (11.1,1.59683) (11.2,1.58839) (11.3,1.82885) (11.4,1.54587) (11.5,1.54952) (11.6,1.55866) (11.7,1.58183) (11.8,1.59432) (11.9,1.62101) (12,1.6388) (12.1,1.79849) (12.2,1.81497) (12.3,1.7037) (12.4,1.73128) (12.5,1.74654) (12.6,1.80269) (12.7,1.77676) (12.8,2.03211) (12.9,1.82485) (13,1.8459) (13.1,1.86389) (13.2,1.88345) (13.3,1.90012) (13.4,1.91828) (13.5,1.94512) (13.6,1.95764) (13.7,1.97915) (13.8,1.99434) (13.9,2.01437) (14,2.046) (14.1,2.12216) (14.2,2.08416) (14.3,2.28318) (14.4,2.12783) (14.5,2.1395) (14.6,2.16081) (14.7,2.17822) (14.8,2.19738) (14.9,2.23218) (15,2.24743) (25,4.33769) (50,10.2865)

	};
	\addlegendentry{\GUS}


%		\addplot (\x, {900}) node[above left]{timeout};		
	\end{semilogyaxis}
\end{scope}


==> figures/PollingSystem_error_late_jt2_qs2_t_5.tex <==
\begin{scope}[local bounding box=scopePLE, shift={($(scopePEE.east)+(1cm, -1.5cm)$)}] 		
	\begin{loglogaxis}[
			x dir=reverse,
			ymin=0,ymax=10000,xmin=1e-10, xmax=1e-03,
			axis y line=left,axis x line=bottom,
			xlabel={   \shortstack{PS-2-2, late, $\choices = 4$, \\ $|S| = 465 $, $\lambda=5.6$, $T=5$}},
			ylabel={},
			height=5cm,
			width=5cm,
			legend style={rounded corners,at={(0.9,0.9)}},
			grid style = {
				dash pattern = on 0.05mm off 1mm,
				line cap = round,
				black,
				line width = 0.5pt
			},
			cycle list name=latelist
		]

		\addplot coordinates {
			(0.001,0.296926) (0.0001,0.940513) (1e-05,3.120200) (1e-06,9.754598) (1e-07,29.234040) (1e-08,91.675459) (1e-09,286.378627) (1e-10,977.544510)  
              } node [pos = 0.6, above left]{\PSS-2};
%		\addlegendentry{\PSS-2}		
		
		\addplot coordinates {
			(0.001,0.275080) (0.0001,0.567868) (1e-05,1.192894) (1e-06,2.530319) (1e-07,5.412250) (1e-08,11.736974) (1e-09,25.170300) (1e-10,54.330123) (1e-11,117.663314) (1e-12,293.155456)  
             } node [pos = 0.6, below right]{\PSS-3};
%		\addlegendentry{\PSS-3}
		
		% \addplot coordinates {
		% 	(0.001,0.017365) (0.0001,0.019221) (1e-05,0.022796) (1e-06,0.025300) (1e-07,0.032475) (1e-08,0.070109) (1e-09,0.304713) (1e-10,2.610888) (1e-11,24.838502) (1e-12,186.603079) 
		% };
		% \addlegendentry{\ASS-1}
		
		% \addplot coordinates {
		% 	(0.001,0.021681) (0.0001,0.024039) (1e-05,0.027498) (1e-06,0.031189) (1e-07,0.034637) (1e-08,0.059585) (1e-09,0.197284) (1e-10,1.572674) (1e-11,14.550294) (1e-12,108.052021) 
		% };
		% \addlegendentry{\ASS-2}

		\addplot coordinates {
			(0.001,0.017365) (0.0001,0.019221) (1e-05,0.022796) (1e-06,0.025300) (1e-07,0.032475) (1e-08,0.059585) (1e-09,0.197284) (1e-10,1.572674) (1e-11,14.550294) (1e-12,108.052021)
             } node [pos = 0.6, above left]{\ASS};
%		\addlegendentry{\ASS}
		
		
		\addplot[unif] coordinates {
			(0.001,0.007945) (0.0001,0.008415) (1e-05,0.006988) (1e-06,0.007221) (1e-07,0.007438) (1e-08,0.006954) (1e-09,0.006822) (1e-10,0.006423) (1e-11,0.006699) (1e-12,0.006380) 
             } node [pos = 0.7, above left]{\GUS};	
%		\addlegendentry{\GUS}
		
%		\addplot (\x, {900});
		
	\end{loglogaxis}
		
\end{scope}

==> figures/PollingSystem_fanout_late_qs2__t_10_e-06.tex <==
\begin{scope}[local bounding box=scopePLF, shift={($(scopePEF.east)+(1cm, -1.5cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10000,xmin=4, xmax=7,
		axis y line=left,axis x line=bottom,
		xlabel={\shortstack{PS-2-x, late, $|S| \in [465,\numprint{85235}]$,\\ $\lambda=[5.6,129.6]$, $T=10,\epsilon=10^{-6}$}},
		ylabel={},
		height=5cm,
		width=5cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
		
		\addplot coordinates {
			(4,305.956428) 
              } node [right]{\PSS-2};
%		\addlegendentry{\PSS-2}		
		
		\addplot coordinates {
			(4,79.008679) 
              } node [right]{\PSS-3};
%		\addlegendentry{\PSS-3}
		
		\addplot coordinates {
			(4,0.253316) (5,7.783852) (6,51.314988) (7,238.001931) 
              } node [pos = 0.4, above left]{\ASS};
%		\addlegendentry{\ASS}%{\ASS-1}
		
		% \addplot coordinates {
		% 	(4,0.326834) (5,10.437570) (6,66.393719) (7,320.796541) 
		% };
		% \addlegendentry{\ASS-2}
		
		\addplot[unif] coordinates {
			(4,0.037283) (5,0.446212) (6,1.741632) (7,7.344354) 
              } node [pos = 0.7, below right]{\GUS};
%		\addlegendentry{\GUS}
		
%		\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}

==> figures/PollingSystem_states_late_jt2_t_5_e-06.tex <==
\begin{scope}[local bounding box=scopePLS, shift={($(scopePES.east)+(1cm, -1.5cm)$)}]  
	\begin{loglogaxis}[
		ymin=0.001,ymax=3200,xmin=456, xmax=1e6,
		axis y line=left,axis x line=bottom,
		xlabel={\hh{todo}},
		ylabel={},
		height=5cm,
		width=5cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
        ]
		
       	\addplot coordinates {
		 (465,2.50866) (2369,18.2404) (10593,96.9513) (44705,538.077) (183585,3119.43) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (465,9.19777) (2369,56.8312) (10593,494.418) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (465,0.038061) (2369,0.104936) (10593,0.372497) (44705,2.59787) (183585,13.7005) (743969,64.029) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (465,0.050168) (2369,0.128584) (10593,0.446986) (44705,3.22015) (183585,16.9946) (743969,78.9134) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (465,0.007413) (2369,0.030897) (10593,0.112857) (44705,0.760189) (183585,4.44514) (743969,20.6486) 
	};
	\addlegendentry{\GUS}
		
%	\addplot (\x, {900});
				
	\end{loglogaxis}
\end{scope}

==> figures/QueuingSystem_Early_Fanout_t=1_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeEF, shift={($(scopeES.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=1000, xmin=2, xmax=7,
		axis y line=left,axis x line=bottom,
		xlabel={fanout},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (2,0.000155) (4,0.002398) (6,0.084838) (8,0.496945) (10,0.651257) (12,1.692431) (14,2.781616) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (2,0.501102) (4,7.763686) (6,47.672016) (8,196.741557) (10,684.778427)
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) node[above left]{timeout};
	\end{semilogyaxis}
\end{scope}


==> figures/QueuingSystem_Early_Precision_t=1.tex <==
\begin{scope}[local bounding box=scopeEE, shift={($(scopeET.south)-(1.6cm, 4cm)$)}]
	\begin{loglogaxis}[
		x dir=reverse,
		ymin=0,ymax=10000,xmin=1e-10, xmax=0.001,
		axis y line=left,axis x line=bottom,
		xlabel={precision},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.001,0.001831) (0.0001,0.005743) (1e-05,0.018006) (1e-06,0.056935) (1e-07,0.181842) (1e-08,0.569191) (1e-09,1.795651) (1e-10,6.004058) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.001,0.000156) (0.0001,0.000153) (1e-05,0.000152) (1e-06,0.000172) (1e-07,0.000179) (1e-08,0.000188) (1e-09,0.000188) (1e-10,0.000199) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.001,0.050776) (0.0001,0.491277) (1e-05,4.923156) (1e-06,49.784530) (1e-07,502.996009) (1e-08,900)  
	};
	\addlegendentry{\ESS-1}


%	\addplot (\x, {900});
	
	\end{loglogaxis}

\end{scope}


==> figures/QueuingSystem_Early_States_t=1_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=10, xmin=26, xmax=500,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]


        	\addplot coordinates {
		 (26,0.000161) (62,0.000403) (112,0.005202) (176,0.006383) (254,0.009463) (346,0.01334) (452,0.020269) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (26,0.63945) (62,1.16337) (112,2.14191) (176,3.45271) (254,5.14121) (346,7.33241) (452,9.72169) 
	};
	\addlegendentry{\ESS-1}



%		\addplot (\x, {900});
	\end{semilogyaxis}
\end{scope}

==> figures/QueuingSystem_Early_Time_t=1.tex <==
\begin{scope}[local bounding box=scopeET] 
	\begin{semilogyaxis}[
		ymin=0.0001,ymax=100, xmin=1, xmax=10,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (1,0.005795) (2,0.016217) (3,0.029742) (4,0.045572) (5,0.064058) (6,0.083629) (7,0.105429) (8,0.128733) (9,0.153308) (10,0.180154) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (1,0.000153) (2,0.000158) (3,0.000162) (4,0.000166) (5,0.000168) (6,0.000170) (7,0.000175) (8,0.000179) (9,0.000184) (10,0.000199) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (1,0.643954) (2,2.004856) (3,4.671060) (4,8.301501) (5,12.453953) (6,17.939429) (7,24.538290) (8,32.841021) (9,40.971120) (10,51.664552) 
	};
	\addlegendentry{\ESS-1}


%		\addplot (\x, {900}) node[above left]{timeout};		
		
	\end{semilogyaxis}
\end{scope}


==> figures/QueuingSystem_Late_Precision_t=1.tex <==
\begin{scope}[local bounding box=scopeLE, shift={($(scopeLT.south)-(1.5cm, 4cm)$)}] 		
	\begin{loglogaxis}[
			x dir=reverse,
			ymin=0,ymax=10000,xmin=1e-10, xmax=1e-03,
			axis y line=left,axis x line=bottom,
			xlabel={precision},
			ylabel={runtime(sec)},
			width=6cm,
			legend style={rounded corners,at={(0.9,0.9)}},
			grid style = {
				dash pattern = on 0.05mm off 1mm,
				line cap = round,
				black,
				line width = 0.5pt
			},
			cycle list name=latelist
		]

                	\addplot coordinates {
		 (0.001,0.133539) (0.0001,0.269728) (1e-05,0.581888) (1e-06,1.249661) (1e-07,2.695423) (1e-08,5.781719) (1e-09,12.429810) (1e-10,26.771824) (1e-11,57.789839) (1e-12,124.389994) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (0.001,0.124053) (0.0001,0.399685) (1e-05,1.261120) (1e-06,3.984745) (1e-07,12.659676) (1e-08,39.975525) (1e-09,126.680732) (1e-10,399.549217) (1e-11,1266.736845) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (0.001,0.010624) (0.0001,0.021581) (1e-05,0.087076) (1e-06,0.382398) (1e-07,3.540583) (1e-08,37.341937) (1e-09,194.010693) (1e-10,406.464731) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (0.001,0.011894) (0.0001,0.019894) (1e-05,0.059161) (1e-06,0.233117) (1e-07,1.633425) (1e-08,15.818981) (1e-09,407.274997) (1e-10,408.815729) (1e-11,409.269545) (1e-12,409.748830) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (0.001,0.014909) (0.0001,0.051628) (1e-05,0.266587) (1e-06,1.527420) (1e-07,11.926979) (1e-08,190.113892) (1e-09,1516.902798) (1e-10,7200) 
	};
	\addlegendentry{\GUS}


		
%		\addplot (\x, {900});
		
	\end{loglogaxis}
		
\end{scope}


==> figures/QueuingSystem_Late_States_t=5_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLS, shift={($(scopeLE.south)-(1.5cm, 4cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10000,xmin=1516, xmax=40000,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]


        	\addplot coordinates {
		 (124,1.31922) (796,10.1896) (3868,56.0425) (16924,337.336) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (124,5.44161) (796,43.092) (3868,247.43) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (124,1.54157) (796,17.9294) (3868,322.955) (16924,1684.73) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (124,0.820327) (796,7.21317) (3868,119.687) (16924,581.487) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (124,1.18993) (796,7.39563) (3868,40.4088) (16924,276.896) 
	};
	\addlegendentry{\GUS}

%	\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}


==> figures/SJS_Early_Fanout_t=1_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeEF, shift={($(scopeES.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=10000, xmin=2, xmax=72,
		axis y line=left,axis x line=bottom,
		xlabel={fanout},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (2,8.6272e-05) (6,0.000317952) (12,0.00162022) (20,0.0077801) (30,0.0372646) (42,0.163823) (56,0.746885) (72,2.66172) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (2,3.435) (6,119.078) (12,1000) (20,1000) (30,1000) (42,1000) (56,1000) (72,1000) 
	};
	\addlegendentry{\ESS-1}


		\addplot (\x, {1000}) node[above left]{timeout};
	\end{semilogyaxis}
\end{scope}

==> figures/SJS_Early_Precision_t=1.tex <==
\begin{scope}[local bounding box=scopeEE, shift={($(scopeET.south)-(1.6cm, 4cm)$)}]
	\begin{loglogaxis}[
		x dir=reverse,
		ymin=0,ymax=10000,xmin=1e-12, xmax=0.001,
		axis y line=left,axis x line=bottom,
		xlabel={precision},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.001,0.000127744) (0.0001,0.000381952) (1e-05,0.00120346) (1e-06,0.00368128) (1e-07,0.0116058) (1e-08,0.0368374) (1e-09,0.116367) (1e-10,0.367014) (1e-11,1.15826) (1e-12,1000) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.001,6.912e-05) (0.0001,6.3488e-05) (1e-05,6.2464e-05) (1e-06,6.9376e-05) (1e-07,7.168e-05) (1e-08,8.1152e-05) (1e-09,7.7056e-05) (1e-10,7.936e-05) (1e-11,0.000123904) (1e-12,0.00013184) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.001,0.00332544) (0.0001,0.0336269) (1e-05,0.343361) (1e-06,3.41055) (1e-07,34.3168) (1e-08,341.82) (1e-09,1000) (1e-10,1000) (1e-11,1000) (1e-12,1000) 
	};
	\addlegendentry{\ESS-1}


	\addplot (\x, {1000});
	
	\end{loglogaxis}

\end{scope}

==> figures/SJS_Early_States_t=1_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeES, shift={($(scopeEE.south)-(1.4cm, 4cm)$)}] 		
	\begin{semilogyaxis}[
		ymin=0,ymax=1000, xmin=9, xmax=300,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (9,8.1664e-05) (19,0.000232448) (33,0.000526592) (51,0.00105446) (73,0.00179328) (99,0.00292762) (129,0.00454298) (163,0.00651622) (201,0.0090729) (243,0.0121958) (289,0.0160589) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (9,4.64432) (19,11.9427) (33,25.2582) (51,46.7504) (73,78.7453) (99,122.659) (129,182.016) (163,258.859) (201,350.175) (243,520.836) (289,1000) 
	};
	\addlegendentry{\ESS-1}


		\addplot (\x, {900});
	\end{semilogyaxis}
\end{scope}

==> figures/SJS_Early_Time_e=1e-04.tex <==
\begin{scope}[local bounding box=scopeET] 
	\begin{semilogyaxis}[
		ymin=0,ymax=10, xmin=0.1, xmax=3.1,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=earlylist
	]
	
        	\addplot coordinates {
		 (0.1,2.7136e-05) (0.2,4.3264e-05) (0.3,7.0912e-05) (0.4,0.000102912) (0.5,0.000139776) (0.6,0.000180992) (0.7,0.000227072) (0.8,0.00027392) (0.9,0.000324864) (1,0.000378112) (1.1,0.000435968) (1.2,0.00049792) (1.3,0.000553472) (1.4,0.00061824) (1.5,0.000693248) (1.6,0.000754688) (1.7,0.000826624) (1.8,0.000913408) (1.9,0.000977664) (2,0.00105267) (2.1,0.00113178) (2.2,0.00121165) (2.3,0.00130048) (2.4,0.00139136) (2.5,0.0014743) (2.6,0.00155878) (2.7,0.0016489) (2.8,0.00173594) (2.9,0.00182707) (3,0.00192691) 
	};
	\addlegendentry{\ESS-2}

	\addplot coordinates {
		 (0.1,9.2416e-05) (0.2,6.3232e-05) (0.3,6.2976e-05) (0.4,6.4256e-05) (0.5,6.2464e-05) (0.6,6.0928e-05) (0.7,6.0928e-05) (0.8,6.0672e-05) (0.9,6.016e-05) (1,5.9648e-05) (1.1,6.5024e-05) (1.2,6.1184e-05) (1.3,5.9904e-05) (1.4,5.9648e-05) (1.5,6.1184e-05) (1.6,6.0672e-05) (1.7,5.9904e-05) (1.8,6.0928e-05) (1.9,6.0672e-05) (2,6.1184e-05) (2.1,6.1184e-05) (2.2,5.9904e-05) (2.3,6.0416e-05) (2.4,6.1184e-05) (2.5,6.0672e-05) (2.6,6.016e-05) (2.7,6.1184e-05) (2.8,6.0672e-05) (2.9,6.1184e-05) (3,6.144e-05) 
	};
	\addlegendentry{\GUS}

	\addplot coordinates {
		 (0.1,0.000357888) (0.2,0.00133734) (0.3,0.00301312) (0.4,0.00552115) (0.5,0.00846336) (0.6,0.0122138) (0.7,0.0171937) (0.8,0.0220506) (0.9,0.0283876) (1,0.0345088) (1.1,0.042836) (1.2,0.0501381) (1.3,0.0598067) (1.4,0.0679206) (1.5,0.0779873) (1.6,0.0883377) (1.7,0.101079) (1.8,0.11321) (1.9,0.126343) (2,0.14074) (2.1,0.153609) (2.2,0.168982) (2.3,0.183368) (2.4,0.19815) (2.5,0.217406) (2.6,0.236978) (2.7,0.252665) (2.8,0.271255) (2.9,0.291928) (3,0.313178) 
	};
	\addlegendentry{\ESS-1}


		\addplot (\x, {900}) node[above left]{timeout};		
		
	\end{semilogyaxis}
\end{scope}

==> figures/SJS_Late_Precision_t=1_23.tex <==
\begin{scope}[local bounding box=scopeLE, shift={($(scopeLT.south)-(1.5cm, 4cm)$)}] 		
	\begin{loglogaxis}[
			x dir=reverse,
			ymin=0,ymax=30,xmin=1e-12, xmax=1e-03,
			axis y line=left,axis x line=bottom,
			xlabel={precision},
			ylabel={runtime(sec)},
			width=6cm,
			legend style={rounded corners,at={(0.9,0.9)}},
			grid style = {
				dash pattern = on 0.05mm off 1mm,
				line cap = round,
				black,
				line width = 0.5pt
			},
			cycle list name=latelist
		]

                	\addplot coordinates {
		 (0.001,0.00306534) (0.0001,0.00660352) (1e-05,0.0140759) (1e-06,0.0303329) (1e-07,0.065195) (1e-08,0.140078) (1e-09,0.302107) (1e-10,0.568078) (1e-11,1.53691) (1e-12,3.31475) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (0.001,0.0022633) (0.0001,0.00718234) (1e-05,0.0226499) (1e-06,0.0718984) (1e-07,0.225767) (1e-08,0.712074) (1e-09,2.25247) (1e-10,7.17259) (1e-11,22.997) (1e-12,72.9147) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (0.001,0.0001024) (0.0001,0.000130048) (1e-05,0.000164352) (1e-06,0.000188672) (1e-07,0.000246528) (1e-08,0.00030336) (1e-09,0.000389376) (1e-10,0.000480768) (1e-11,0.000616448) (1e-12,0.000870912) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (0.001,0.00033536) (0.0001,0.000388352) (1e-05,0.000474624) (1e-06,0.000608768) (1e-07,0.000744448) (1e-08,0.000945664) (1e-09,0.00117632) (1e-10,0.00148352) (1e-11,0.00184806) (1e-12,0.00229402) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (0.001,0.000112896) (0.0001,0.000108544) (1e-05,0.000107776) (1e-06,0.00012032) (1e-07,0.000120064) (1e-08,0.000140032) (1e-09,0.00013312) (1e-10,0.00013312) (1e-11,0.000145664) (1e-12,0.000145664) 
	};
	\addlegendentry{\GUS}


		
		\addplot (\x, {900});
		
	\end{loglogaxis}
		
\end{scope}

==> figures/SJS_Late_States_t=1_e=1e-06.tex <==
\begin{scope}[local bounding box=scopeLS, shift={($(scopeLE.south)-(1.5cm, 4cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=1,xmin=9, xmax=300,
		axis y line=left,axis x line=bottom,
		xlabel={state space},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
		
        	\addplot coordinates {
		 (9,0.00171597) (19,0.00601856) (33,0.0124124) (51,0.0226691) (73,0.0371392) (99,0.0508219) (129,0.074987) (163,0.115784) (201,0.155787) (243,0.190119) (289,0.245659) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (9,0.00420557) (19,0.010518) (33,0.0231424) (51,0.0402796) (73,0.0680842) (99,0.107218) (129,0.165915) (163,0.224373) (201,0.305116) (243,0.398056) (289,0.501619) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (9,0.000141568) (19,0.000241408) (33,0.000474368) (51,0.000582912) (73,0.0009344) (99,0.00133478) (129,0.00172416) (163,0.00220314) (201,0.00263347) (243,0.00294758) (289,0.00338381) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (9,0.000310784) (19,0.00038528) (33,0.000466944) (51,0.000644096) (73,0.000883712) (99,0.00116454) (129,0.00153779) (163,0.00202138) (201,0.00256896) (243,0.00309504) (289,0.00375987) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (9,6.0928e-05) (19,0.000129024) (33,0.000260608) (51,0.000491776) (73,0.000828928) (99,0.00133197) (129,0.00194458) (163,0.00282829) (201,0.00380211) (243,0.00486938) (289,0.00606131) 
	};
	\addlegendentry{\GUS}


		\addplot (\x, {900});
				
	\end{semilogyaxis}
\end{scope}

==> figures/SJS_Late_Time_e=1e-06_23.tex <==
\begin{scope}[local bounding box=scopeLT, shift={($(scopeET.east)+(2cm, -1.5cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=1,xmin=0.1, xmax=3.1,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(.9,.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
        	\addplot coordinates {
		 (0.1,0.0017751) (0.2,0.00335181) (0.3,0.00659046) (0.4,0.00807962) (0.5,0.0108019) (0.6,0.0139341) (0.7,0.0166994) (0.8,0.0198756) (0.9,0.0232612) (1,0.0266519) (1.1,0.0301819) (1.2,0.0401564) (1.3,0.0441393) (1.4,0.0418186) (1.5,0.0457183) (1.6,0.04979) (1.7,0.0537743) (1.8,0.0649556) (1.9,0.0622607) (2,0.0760202) (2.1,0.0710807) (2.2,0.0864801) (2.3,0.0801293) (2.4,0.0972403) (2.5,0.102419) (2.6,0.107846) (2.7,0.11352) (2.8,0.119064) (2.9,0.124736) (3,0.130785) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (0.1,0.00229811) (0.2,0.00641306) (0.3,0.0115727) (0.4,0.0183158) (0.5,0.025931) (0.6,0.0331745) (0.7,0.0420201) (0.8,0.0511457) (0.9,0.0624433) (1,0.0715794) (1.1,0.0851377) (1.2,0.0949005) (1.3,0.106356) (1.4,0.119161) (1.5,0.132051) (1.6,0.148435) (1.7,0.160621) (1.8,0.176346) (1.9,0.190281) (2,0.202246) (2.1,0.220786) (2.2,0.235832) (2.3,0.25285) (2.4,0.275531) (2.5,0.286906) (2.6,0.303078) (2.7,0.321305) (2.8,0.342278) (2.9,0.355952) (3,0.378357) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (0.1,2.9696e-05) (0.2,5.6832e-05) (0.3,5.76e-05) (0.4,9.088e-05) (0.5,9.0368e-05) (0.6,0.00012416) (0.7,0.000124672) (0.8,0.000159232) (0.9,0.000192) (1,0.000192) (1.1,0.000227072) (1.2,0.00022912) (1.3,0.000272896) (1.4,0.000303872) (1.5,0.000305408) (1.6,0.000341504) (1.7,0.000351744) (1.8,0.0003776) (1.9,0.000379392) (2,0.000403712) (2.1,0.000420096) (2.2,0.00045312) (2.3,0.000453376) (2.4,0.000489472) (2.5,0.000531456) (2.6,0.000527872) (2.7,0.000561664) (2.8,0.000565248) (2.9,0.000599296) (3,0.000601856) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (0.1,6.3744e-05) (0.2,0.000113152) (0.3,0.000173312) (0.4,0.000212224) (0.5,0.00027776) (0.6,0.000345856) (0.7,0.000409088) (0.8,0.000447744) (0.9,0.000521472) (1,0.000590848) (1.1,0.000661504) (1.2,0.000735232) (1.3,0.000751104) (1.4,0.000845568) (1.5,0.000920576) (1.6,0.000995584) (1.7,0.00104192) (1.8,0.0010729) (1.9,0.00118374) (2,0.00122189) (2.1,0.00128512) (2.2,0.00136858) (2.3,0.00140928) (2.4,0.0015145) (2.5,0.00155699) (2.6,0.0016087) (2.7,0.00168499) (2.8,0.00174234) (2.9,0.00180966) (3,0.00190336) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (0.1,0.000456448) (0.2,0.000377088) (0.3,0.000361984) (0.4,0.000360448) (0.5,0.000374016) (0.6,0.000425472) (0.7,0.000361728) (0.8,0.000361472) (0.9,0.000364544) (1,0.000366336) (1.1,0.0003648) (1.2,0.000386816) (1.3,0.000373504) (1.4,0.000374528) (1.5,0.000377344) (1.6,0.00038272) (1.7,0.000366336) (1.8,0.000365824) (1.9,0.000383488) (2,0.00037632) (2.1,0.000377088) (2.2,0.000377088) (2.3,0.000376832) (2.4,0.000388864) (2.5,0.000379392) (2.6,0.00038016) (2.7,0.00038016) (2.8,0.000380416) (2.9,0.000379904) (3,0.000382208) 
	};
	\addlegendentry{\GUS}


		\addplot (\x, {900}) node[above left]{timeout};		
	\end{semilogyaxis}
\end{scope}

==> figures/SJS_Late_Time_e=1e-06_35.tex <==
\begin{scope}[local bounding box=scopeLT, shift={($(scopeET.east)+(2cm, -1.5cm)$)}] 
	\begin{semilogyaxis}[
		ymin=0,ymax=200,xmin=0.1, xmax=3.1,
		axis y line=left,axis x line=bottom,
		xlabel={time bound},
		ylabel={runtime(sec)},
		width=6cm,
		legend style={rounded corners,at={(0.9,0.9)}},
		grid style = {
			dash pattern = on 0.05mm off 1mm,
			line cap = round,
			black,
			line width = 0.5pt
		},
		cycle list name=latelist
	]
        	\addplot coordinates {
		 (0.1,0.575384) (0.2,1.44684) (0.3,2.48944) (0.4,3.64445) (0.5,4.88592) (0.6,6.25058) (0.7,7.66453) (0.8,9.16142) (0.9,10.6784) (1,12.325) (1.1,13.9533) (1.2,15.6821) (1.3,17.3814) (1.4,19.3035) (1.5,21.0591) (1.6,22.9428) (1.7,24.8623) (1.8,26.8789) (1.9,28.8446) (2,30.8484) (2.1,32.8166) (2.2,35.0392) (2.3,37.1735) (2.4,39.3476) (2.5,41.4061) (2.6,43.7686) (2.7,46.0591) (2.8,48.2542) (2.9,50.4144) (3,52.8915) 
	};
	\addlegendentry{\PSS-3}

	\addplot coordinates {
		 (0.1,0.993759) (0.2,3.00886) (0.3,5.53634) (0.4,8.50897) (0.5,11.9015) (0.6,15.635) (0.7,19.7435) (0.8,24.0179) (0.9,29.0569) (1,33.5897) (1.1,38.5998) (1.2,44.0712) (1.3,49.7198) (1.4,55.2716) (1.5,61.4476) (1.6,67.6919) (1.7,73.9459) (1.8,80.6997) (1.9,87.1523) (2,94.1671) (2.1,101.461) (2.2,109.14) (2.3,116.098) (2.4,123.41) (2.5,131.458) (2.6,139.225) (2.7,147.301) (2.8,155.33) (2.9,163.744) (3,173.033) 
	};
	\addlegendentry{\PSS-2}

	\addplot coordinates {
		 (0.1,0.0123697) (0.2,0.0227338) (0.3,0.0305915) (0.4,0.0322703) (0.5,0.0374684) (0.6,0.0411287) (0.7,0.0439767) (0.8,0.0439099) (0.9,0.0499538) (1,0.0561533) (1.1,0.0592932) (1.2,0.0654454) (1.3,0.0718085) (1.4,0.0748321) (1.5,0.081121) (1.6,0.0871739) (1.7,0.0904645) (1.8,0.0966331) (1.9,0.0997903) (2,0.10614) (2.1,0.112112) (2.2,0.115394) (2.3,0.121486) (2.4,0.124763) (2.5,0.130989) (2.6,0.13408) (2.7,0.140342) (2.8,0.143771) (2.9,0.149636) (3,0.152824) 
	};
	\addlegendentry{\ASS-1}

	\addplot coordinates {
		 (0.1,0.0082153) (0.2,0.0145807) (0.3,0.0214321) (0.4,0.0280228) (0.5,0.0345892) (0.6,0.043255) (0.7,0.0500101) (0.8,0.056491) (0.9,0.0649748) (1,0.0717271) (1.1,0.0815585) (1.2,0.0869834) (1.3,0.0937439) (1.4,0.100348) (1.5,0.108746) (1.6,0.115668) (1.7,0.122619) (1.8,0.129097) (1.9,0.137442) (2,0.144343) (2.1,0.150717) (2.2,0.157402) (2.3,0.164036) (2.4,0.174127) (2.5,0.179274) (2.6,0.186088) (2.7,0.192266) (2.8,0.198761) (2.9,0.205289) (3,0.21147) 
	};
	\addlegendentry{\ASS-2}

	\addplot coordinates {
		 (0.1,0.0159035) (0.2,0.0161244) (0.3,0.0162591) (0.4,0.0163901) (0.5,0.0165519) (0.6,0.0166659) (0.7,0.0168177) (0.8,0.0170376) (0.9,0.0171932) (1,0.017377) (1.1,0.0175455) (1.2,0.0177408) (1.3,0.0178941) (1.4,0.0180759) (1.5,0.018175) (1.6,0.0183025) (1.7,0.0186586) (1.8,0.018665) (1.9,0.0187395) (2,0.018946) (2.1,0.0190979) (2.2,0.0192492) (2.3,0.0193567) (2.4,0.0194875) (2.5,0.0197217) (2.6,0.0198252) (2.7,0.0199813) (2.8,0.020151) (2.9,0.0203169) (3,0.0205612) 
	};
	\addlegendentry{\GUS}


		\addplot (\x, {900}) node[above left]{timeout};		
	\end{semilogyaxis}
\end{scope}
